CLINICSUM: Utilizing Language Models for Generating Clinical Summaries from Patient-Doctor Conversations

This paper presents ClinicSum, a novel framework designed to automatically generate clinical summaries from patient-doctor conversations. It utilizes a two-module architecture: a retrieval-based filtering module that extracts Subjective, Objective, Assessment, and Plan (SOAP) information from conversation transcripts, and an inference module powered by fine-tuned Pre-trained Language Models (PLMs), which leverage the extracted SOAP data to generate abstracted clinical summaries. To fine-tune the PLM, we created a training dataset of consisting 1,473 conversations-summaries pair by consolidating two publicly available datasets, FigShare and MTS-Dialog, with ground truth summaries validated by Subject Matter Experts (SMEs). ClinicSum's effectiveness is evaluated through both automatic metrics (e.g., ROUGE, BERTScore) and expert human assessments. Results show that ClinicSum outperforms state-of-the-art PLMs, demonstrating superior precision, recall, and F-1 scores in automatic evaluations and receiving high preference from SMEs in human assessment, making it a robust solution for automated clinical summarization.

==> HImanshu_method.tex <==
The DialogSum architecture is designed to generate concise semi-structured SOAP summaries from transcribed clinical dialogues. It operates in two distinct phases: retriever-based filtering and inference. In the first phase, unnecessary information is removed from the transcribed text, setting the stage for the second phase, where the refined information is passed to a fine-tuned PLM adept at generating SOAP summaries.

% \subsection{Retriever Based Filtering}
% The first module in our \framework framework is designed to systematically process doctor-patient conversation transcripts to extract relevant information necessary for generating SOAP clinical summaries.


% Initially, the module receives the raw transcripts from the interactions between doctors and patients. These transcripts are then subjected to a sentence splitting procedure. This procedure employs regular expressions to detect sentence boundaries, specifically targeting periods and question marks. As a result, each identified sentence is isolated and treated as a distinct chunk for further processing. Next, these chunks undergo an embedding generation process. This step involves applying embedding models to transform the textual chunks into corresponding embedding vectors. These embedded vectors encapsulate the semantic content of the sentences, making them suitable for further analysis. Subsequently, an advanced retriever mechanism analyzes the embedded chunks using a structured prompt designed to extract SOAP (Subjective, Objective, Assessment, and Plan) information. The retriever processes the chunks, extracting clinically relevant vectors, which are then filtered to remove noise and irrelevant data, ensuring the retention of pertinent information.

% The filtered vectors are converted back into coherent text through a process called text reconstruction. The reconstructed texts are concatenated to form a combined text document, serving as input context for the inference module.




\subsection{Inference}

\subsubsection{Fine-tuning}

% \subsubsection{Generation}
% The input to the inference module includes the patient context, derived from the retriever-based filtering module, and a structured prompt. This prompt instructs a LLM to generate clinical summaries in a zero-shot setting based on the provided context. The inference module leverages the fine-tuned LLM generator, which has been pre-trained to produce SOAP summaries. By processing the structured prompt and patient context, the model generates a coherent and comprehensive clinical SOAP summary, ensuring the extraction of clinically relevant information from patient context. 

% \framework is effective in zero-shot settings due to the fine-tuning of the LLM, allowing it to generalize well to new, unseen patient contexts without requiring additional training data.

\subsection{Retriever Based Filtering}
In the first phase, we've discussed how each sentence is treated as an individual chunk, which limits the scope of information to that chunk rather than dispersing it across the surrounding text. These chunks are then converted into embeddings using an embedding model, allowing a hybrid retriever to search through the text efficiently. Next, we feed a carefully crafted prompt to the retriever, guiding it to filter out chunks that do not align with the required context. The resulting chunks are then decoded and reconstructed into a coherent patient context, which forms the basis for the next phase.

\subsection{Generation}
With the patient context prepared, the inference module comes into play. This module receives the patient context from the retriever-based filtering and uses it alongside a structured prompt to instruct an LLM to generate clinical summaries. The fine-tuned LLM, pre-trained specifically for SOAP summary generation, processes the prompt and context to produce a coherent and relevant SOAP summary. This ensures that the summary accurately reflects the most clinically pertinent information extracted from the patient context, preparing for the final output of the summary.

\subsection{Illustration}
Imagine if we had the following transcribed text:

\textit{“Good morning doctor. Good morning, what brings you here. I've had a cough for about six months, recently noticed some blood. Is it a dry or wet cough? Mostly dry, but lately with some blood. How much blood are you coughing up? About two or three teaspoons a day. Any shortness of breath or chest pain? Shortness of breath, especially with activity, but no chest pain. Any recent weight loss? Yes, around ten to fifteen pounds in the last two months. Do you smoke? Yes, half a pack a day, but I've been cutting down. We need to do a chest X-ray and sputum test. Lung cancer is a concern given your symptoms and smoking history. That makes sense, thank you. We'll proceed with those tests and follow up. Take care.``}

Then, in the retriever-based filtering, we first split the entire block of text into sentences.

\textit{convo} = \{

    \textit{“Good morning doctor.``,}
     
    \textit{“Good morning, what brings you here.``,}

    \textit{"I've had a cough for about six months, recently noticed some blood.``,}
    
    \textit{"Is it a dry or wet cough?``,}
    
    \textit{"Mostly dry, but lately with some blood.``,}
    
    \textit{"How much blood are you coughing up?``,}
    
    \textit{"About two or three teaspoons a day.``,}
    
    \textit{"Any shortness of breath or chest pain?``,}
    
    \textit{"Shortness of breath, especially with activity, but no chest pain.``,}
    
    \textit{"Any recent weight loss?``,}
    
    \textit{"Yes, around ten to fifteen pounds in the last two months.``,}
    
    \textit{"Do you smoke?``,}
    
    \textit{"Yes, half a pack a day, but I've been cutting down.``,}
    
    \textit{"We need to do a chest X-ray and sputum test. Lung cancer is a concern given your symptoms and smoking history.``,}
    
    \textit{"That makes sense, thank you.``,}
    
    \textit{"We'll proceed with those tests and follow up.``}

\}


Now we embed all the chunks,

\begin{equation*}
    convo = \{E(t_i)\}_{i = 1}^{n}
\end{equation*}

This expression represents the entire conversation as the set of vector embeddings $E(t_i)$ for each line $t_i$, with $i$ ranging from 1 to n.

We now pass it to the hybrid retriever, where the symantic meaning is taken care of by the dense retriever and the syntactic information is taken care of by the sparse retriever. The retriever removes all the unnecessary information with respect to the prompt that is being passed, after which we decode each chunk and concatenate them to reconstruct a subset of the initial text that only contains the information that is required.

\textit{"I've had a cough for about six months, recently noticed some blood. Is it a dry or wet cough? Mostly dry, but lately with some blood. How much blood are you coughing up? About two or three teaspoons a day. Any shortness of breath or chest pain? Shortness of breath, especially with activity, but no chest pain. Any recent weight loss? Yes, around ten to fifteen pounds in the last two months. Do you smoke? Yes, half a pack a day, but I've been cutting down. We need to do a chest X-ray and sputum test. Lung cancer is a concern given your symptoms and smoking history. That makes sense, thank you.``}

In the generation phase, the pure information extracted from the text in phase 1 will be passed to a fine-tuned LLM, which can generate SOAP notes,

\begin{enumerate}
    \item \textbf{Subjective:}
    \begin{enumerate}
        \item \textbf{Chief Complaint:} Persistent cough for six months with recent hemoptysis.
        \item \textbf{History of Present Illness:} The patient reports having a cough for approximately six months. Initially, the cough was dry, but in recent weeks, they have noticed blood in the sputum. They estimate coughing up about two to three teaspoons of blood daily. The cough is constant and associated with shortness of breath, especially during physical activity. No chest pain is noted. The patient has experienced a weight loss of 10-15 pounds over the last two months. They have a history of smoking, currently half a pack per day, down from two packs per day.
    \end{enumerate}
    
    \item \textbf{Objective:}
    \begin{enumerate}
        \item \textbf{General:} Patient appears concerned but is cooperative and oriented.
        \item \textbf{Respiratory:} Persistent cough with reported hemoptysis. No audible wheezing or rales noted at this time.
        \item \textbf{Vitals:} (Not provided but necessary for full evaluation.)
    \end{enumerate}
    
    \item \textbf{Assessment:}
    \begin{enumerate}
        \item \textbf{Chronic Cough with Hemoptysis:} Differential diagnoses include but are not limited to lung cancer, chronic bronchitis, or a pulmonary infection. Given the patient's significant smoking history and recent weight loss, lung cancer is a primary concern.
    \end{enumerate}
    
    \item \textbf{Plan:}
    \begin{enumerate}
        \item \textbf{Diagnostic Tests:}
        \begin{enumerate}
            \item Order a chest X-ray to assess for any masses, lesions, or other abnormalities.
            \item Collect a sputum sample for cytology to check for malignant cells.
        \end{enumerate}
        \item \textbf{Smoking Cessation:}
        \begin{enumerate}
            \item Discuss smoking cessation strategies, including pharmacotherapy options such as Champix (varenicline).
        \end{enumerate}
        \item \textbf{Follow-Up:}
        \begin{enumerate}
            \item Schedule a follow-up appointment to review test results and discuss further diagnostic procedures if needed, such as a CT scan or biopsy, depending on initial findings.
        \end{enumerate}
    \end{enumerate}
    
    \item \textbf{Patient Education:}
    \begin{enumerate}
        \item Educate the patient on the importance of early detection and the risks associated with continued smoking. Provide resources for smoking cessation support.
    \end{enumerate}
    
    \item \textbf{Next Steps:}
    \begin{enumerate}
        \item Await the results of the chest X-ray and sputum cytology. Depending on findings, further imaging or referral to a pulmonologist may be necessary.
    \end{enumerate}
\end{enumerate}



\[
\begin{aligned}
C_p = (& \text{Demographics } (D: \text{42-year-old white female}), \\
&  (MH: \text{Asthma, Allergic Rhinitis, Cervical Dysplasia, Premenstrual Dysphoric Disorder, Stress Incontinence}), \\
&  (M: \text{Proventil, Allegra, Flovent, Fluoxetine, Flonase}), \\
& (Dx: \text{Vital signs within normal range, normal physical exam except for vaginal discharge}), \\
&  (FH, SH: \text{Married, Nonsmoker}), \\
&  (LC: \text{Potential allergen exposure due to husband's occupation}), \\
&  (TP: \text{Asthma management with Flovent, consider Advair/Singulair, follow-up in one month,} \\
& \text{restart Allegra and Flonase, Fluoxetine for PMDD, repeat UA for hematuria, Pap smear, mammogram, calcium/vitamin D supplements})
)
\end{aligned}
\]

==> Illustration.tex <==
Imagine if we had the following diarized patient-doctor conversation, 

\begin{tcolorbox}[colback=blue!5!white,colframe=blue!75!black,title=Diarized Patient-Doctor Conversation, breakable]
\footnotesize
\textbf{P:} Good morning, doctor. \\
\textbf{D:} Good morning. What brings you here? \\
\textbf{P:} I've had a cough for about six months. Recently noticed some blood. \\
\textbf{D:} Is it a dry or wet cough? \\
\textbf{P:} Mostly dry. But lately with some blood. \\
\textbf{D:} How much blood are you coughing up? \\
\textbf{P:} About two or three teaspoons a day. \\
\textbf{D:} Any shortness of breath or chest pain? \\
\textbf{P:} Shortness of breath, especially with activity. But no chest pain. \\
\textbf{D:} Any recent weight loss? \\
\textbf{P:} Yes, around ten to fifteen pounds in the last two months. \\
\textbf{D:} Do you smoke? \\
\textbf{P:} Yes, half a pack a day. I've been cutting down. \\
\textbf{D:} We need to do a chest X-ray and sputum test. Lung cancer is a concern given your symptoms and smoking history. \\
\textbf{P:} That makes sense. Thank you. \\
\textbf{D:} We'll proceed with those tests and follow up. Take care. \\
\textbf{P:} Thank you, doctor. Goodbye. \\
\textbf{D:} Goodbye and take care. \\
\end{tcolorbox}

This diarized text can simply be converted to patient-doctor transcribed text like this,

\begin{tcolorbox}[colback=blue!5!white,colframe=blue!75!black,title=Transcribed Patient-Doctor Conversation, breakable]
\footnotesize
Good morning, doctor. Good morning. What brings you here? I've had a cough for about six months. Recently noticed some blood. Is it a dry or wet cough? Mostly dry. But lately with some blood. How much blood are you coughing up? About two or three teaspoons a day. Any shortness of breath or chest pain? Shortness of breath, especially with activity, but no chest pain. Any recent weight loss? Yes, around ten to fifteen pounds in the last two months. Do you smoke? Yes, half a pack a day. I've been cutting down. We need to do a chest X-ray and sputum test. Lung cancer is a concern given your symptoms and smoking history. That makes sense. Thank you. We'll proceed with those tests and follow up. Take care. Thank you, doctor. Goodbye. Goodbye and take care.
\end{tcolorbox}


\subsection*{Retriever Based Filtering}

\textbf{Splitting}

In the first step of retriever-based filtering, we split the transcribed text into individual sentences. This approach ensures that each sentence is processed independently, so the information is contained within each sentence without being spread across multiple chunks. As a result, each chunk makes sense on its own, independent of the others, when received by the LLM.

\begin{tcolorbox}[colback=blue!5!white,colframe=blue!75!black,title=Sentence-wise Splitted Chunked Patient-Doctor Conversation, breakable]
\footnotesize
\textbf{Chunk 1}: Good morning, doctor. \\
\textbf{Chunk 2}: Good morning. \\
\textbf{Chunk 3}: What brings you here? \\
\textbf{Chunk 4}: I've had a cough for about six months. \\
\textbf{Chunk 5}: Recently noticed some blood. \\
\textbf{Chunk 6}: Is it a dry or wet cough? \\
\textbf{Chunk 7}: Mostly dry. \\
\textbf{Chunk 8}: But lately with some blood. \\
\textbf{Chunk 9}: How much blood are you coughing up? \\
\textbf{Chunk 10}: About two or three teaspoons a day. \\
\textbf{Chunk 11}: Any shortness of breath or chest pain? \\
\textbf{Chunk 12}: Shortness of breath, especially with activity. \\
\textbf{Chunk 13}: But no chest pain. \\
\textbf{Chunk 14}: Any recent weight loss? \\
\textbf{Chunk 15}: Yes, around ten to fifteen pounds in the last two months. \\
\textbf{Chunk 16}: Do you smoke? \\
\textbf{Chunk 17}: Yes, half a pack a day. \\
\textbf{Chunk 18}: I've been cutting down. \\
\textbf{Chunk 19}: We need to do a chest X-ray and sputum test. \\
\textbf{Chunk 20}: Lung cancer is a concern given your symptoms and smoking history. \\
\textbf{Chunk 21}: That makes sense. \\
\textbf{Chunk 22}: Thank you. \\
\textbf{Chunk 23}: We'll proceed with those tests and follow up. \\
\textbf{Chunk 24}: Take care. \\
\textbf{Chunk 25}: Thank you, doctor. \\
\textbf{Chunk 26}: Goodbye. \\
\textbf{Chunk 27}: Goodbye and take care.
\end{tcolorbox}

\textbf{Indexing}

After splitting, we embedded each chunk for retrieval handling.

\begin{tcolorbox}[colback=blue!5!white,colframe=blue!75!black,title=Embedded Patient-Doctor Conversation, breakable]
\footnotesize
\textbf{Chunk 1:} \textit{Good morning, doctor.} \\
\textbf{Embedded Format:} \\
\begin{minipage}[t]{0.45\textwidth}
\footnotesize
\begin{verbatim}
[0.123, -0.567, 0.910...]
\end{verbatim}
\end{minipage}

\textbf{Chunk 2:} \textit{Good morning.} \\
\textbf{Embedded Format:} \\
\begin{minipage}[t]{0.45\textwidth}
\footnotesize
\begin{verbatim}
[0.234, -0.678, 0.821...]
\end{verbatim}
\end{minipage}

\textbf{Chunk 3:} \textit{What brings you here?} \\
\textbf{Embedded Format:} \\
\begin{minipage}[t]{0.45\textwidth}
\footnotesize
\begin{verbatim}
[0.345, -0.789, 0.732...]
\end{verbatim}
\end{minipage}

\textbf{Chunk 4:} \textit{I've had a cough for about six months.} \\
\textbf{Embedded Format:} \\
\begin{minipage}[t]{0.45\textwidth}
\footnotesize
\begin{verbatim}
[0.456, -0.890, 0.643...]
\end{verbatim}
\end{minipage}

\textbf{Chunk 5:} \textit{Recently noticed some blood.} \\
\textbf{Embedded Format:} \\
\begin{minipage}[t]{0.45\textwidth}
\footnotesize
\begin{verbatim}
[0.567, -0.901, 0.554...]
\end{verbatim}
\end{minipage}

\textbf{Chunk 6:} \textit{Is it a dry or wet cough?} \\
\textbf{Embedded Format:} \\
\begin{minipage}[t]{0.45\textwidth}
\footnotesize
\begin{verbatim}
[0.678, -0.912, 0.465...]
\end{verbatim}
\end{minipage}

\textbf{Chunk 7:} \textit{Mostly dry.} \\
\textbf{Embedded Format:} \\
\begin{minipage}[t]{0.45\textwidth}
\footnotesize
\begin{verbatim}
[0.789, -0.923, 0.376...]
\end{verbatim}
\end{minipage}

\textbf{Chunk 8:} \textit{But lately with some blood.} \\
\textbf{Embedded Format:} \\
\begin{minipage}[t]{0.45\textwidth}
\footnotesize
\begin{verbatim}
[0.890, -0.934, 0.287...]
\end{verbatim}
\end{minipage}

\textbf{Chunk 9:} \textit{How much blood are you coughing up?} \\
\textbf{Embedded Format:} \\
\begin{minipage}[t]{0.45\textwidth}
\footnotesize
\begin{verbatim}
[0.901, -0.945, 0.198...]
\end{verbatim}
\end{minipage}

\textbf{Chunk 10:} \textit{About two or three teaspoons a day.} \\
\textbf{Embedded Format:} \\
\begin{minipage}[t]{0.45\textwidth}
\footnotesize
\begin{verbatim}
[0.012, -0.956, 0.109...]
\end{verbatim}
\end{minipage}

\textbf{Chunk 11:} \textit{Any shortness of breath or chest pain?} \\
\textbf{Embedded Format:} \\
\begin{minipage}[t]{0.45\textwidth}
\footnotesize
\begin{verbatim}
[0.123, -0.967, 0.210...]
\end{verbatim}
\end{minipage}

\textbf{Chunk 12:} \textit{Shortness of breath, especially with activity.} \\
\textbf{Embedded Format:} \\
\begin{minipage}[t]{0.45\textwidth}
\footnotesize
\begin{verbatim}
[0.234, -0.978, 0.321...]
\end{verbatim}
\end{minipage}

\textbf{Chunk 13:} \textit{But no chest pain.} \\
\textbf{Embedded Format:} \\
\begin{minipage}[t]{0.45\textwidth}
\footnotesize
\begin{verbatim}
[0.345, -0.989, 0.432...]
\end{verbatim}
\end{minipage}

\textbf{Chunk 14:} \textit{Any recent weight loss?} \\
\textbf{Embedded Format:} \\
\begin{minipage}[t]{0.45\textwidth}
\footnotesize
\begin{verbatim}
[0.456, -0.990, 0.543...]
\end{verbatim}
\end{minipage}

\textbf{Chunk 15:} \textit{Yes, around ten to fifteen pounds in the last two months.} \\
\textbf{Embedded Format:} \\
\begin{minipage}[t]{0.45\textwidth}
\footnotesize
\begin{verbatim}
[0.567, -0.991, 0.654...]
\end{verbatim}
\end{minipage}

\textbf{Chunk 16:} \textit{Do you smoke?} \\
\textbf{Embedded Format:} \\
\begin{minipage}[t]{0.45\textwidth}
\footnotesize
\begin{verbatim}
[0.678, -0.992, 0.765...]
\end{verbatim}
\end{minipage}

\textbf{Chunk 17:} \textit{Yes, half a pack a day.} \\
\textbf{Embedded Format:} \\
\begin{minipage}[t]{0.45\textwidth}
\footnotesize
\begin{verbatim}
[0.789, -0.993, 0.876...]
\end{verbatim}
\end{minipage}

\textbf{Chunk 18:} \textit{I've been cutting down.} \\
\textbf{Embedded Format:} \\
\begin{minipage}[t]{0.45\textwidth}
\footnotesize
\begin{verbatim}
[0.890, -0.994, 0.987...]
\end{verbatim}
\end{minipage}

\textbf{Chunk 19:} \textit{We need to do a chest X-ray and sputum test.} \\
\textbf{Embedded Format:} \\
\begin{minipage}[t]{0.45\textwidth}
\footnotesize
\begin{verbatim}
[0.901, -0.995, 0.098...]
\end{verbatim}
\end{minipage}

\textbf{Chunk 20:} \textit{Lung cancer is a concern given your symptoms and smoking history.} \\
\textbf{Embedded Format:} \\
\begin{minipage}[t]{0.45\textwidth}
\footnotesize
\begin{verbatim}
[0.012, -0.996, 0.209...]
\end{verbatim}
\end{minipage}

\textbf{Chunk 21:} \textit{That makes sense.} \\
\textbf{Embedded Format:} \\
\begin{minipage}[t]{0.45\textwidth}
\footnotesize
\begin{verbatim}
[0.123, -0.997, 0.320...]
\end{verbatim}
\end{minipage}

\textbf{Chunk 22:} \textit{Thank you.} \\
\textbf{Embedded Format:} \\
\begin{minipage}[t]{0.45\textwidth}
\footnotesize
\begin{verbatim}
[0.125, -0.897, 0.356...]
\end{verbatim}
\end{minipage}

\textbf{Chunk 23:} \textit{We'll proceed with those tests and follow up.} \\
\textbf{Embedded Format:} \\
\begin{minipage}[t]{0.45\textwidth}
\footnotesize
\begin{verbatim}
[0.234, -0.998, 0.431...]
\end{verbatim}
\end{minipage}

\textbf{Chunk 24:} \textit{Take care.} \\
\textbf{Embedded Format:} \\
\begin{minipage}[t]{0.45\textwidth}
\footnotesize
\begin{verbatim}
[0.345, -0.999, 0.542...]
\end{verbatim}
\end{minipage}

\textbf{Chunk 25:} \textit{Thank you, doctor.} \\
\textbf{Embedded Format:} \\
\begin{minipage}[t]{0.45\textwidth}
\footnotesize
\begin{verbatim}
[-0.345, -0.934, 0.542...]
\end{verbatim}
\end{minipage}

\textbf{Chunk 26:} \textit{Goodbye.} \\
\textbf{Embedded Format:} \\
\begin{minipage}[t]{0.45\textwidth}
\footnotesize
\begin{verbatim}
[0.356, -0.999, 0.532...]
\end{verbatim}
\end{minipage}

\textbf{Chunk 27:} \textit{Goodbye and take care.} \\
\textbf{Embedded Format:} \\
\begin{minipage}[t]{0.45\textwidth}
\footnotesize
\begin{verbatim}
[0.344, -0.999, -0.742...]
\end{verbatim}
\end{minipage}

\vspace{5mm}
\textit{Note: The embedding values shown are illustrative representations and not actual embedding values.}
\end{tcolorbox}

\textbf{Retrieval}


Now, we embed the retriever query and use it to identify the relevant embedded chunks for generating SOAP notes.

\begin{tcolorbox}[colback=blue!5!white,colframe=blue!75!black,title=Retrived and Rearranged Chunks, breakable]
\footnotesize

\textbf{Retrieved Chunk 1: } \\
\begin{minipage}[t]{0.45\textwidth}
\footnotesize
\begin{verbatim}
[0.456, -0.890, 0.643...]
\end{verbatim}
\end{minipage}

\textbf{Retrieved Chunk 2: } \\
\begin{minipage}[t]{0.45\textwidth}
\footnotesize
\begin{verbatim}
[0.567, -0.901, 0.554...]
\end{verbatim}
\end{minipage}

\textbf{Retrieved Chunk 3: } \\
\begin{minipage}[t]{0.45\textwidth}
\footnotesize
\begin{verbatim}
[0.678, -0.912, 0.465...]
\end{verbatim}
\end{minipage}

\textbf{Retrieved Chunk 4: } \\
\begin{minipage}[t]{0.45\textwidth}
\footnotesize
\begin{verbatim}
[0.789, -0.923, 0.376...]
\end{verbatim}
\end{minipage}

\textbf{Retrieved Chunk 5: } \\
\begin{minipage}[t]{0.45\textwidth}
\footnotesize
\begin{verbatim}
[0.890, -0.934, 0.287...]
\end{verbatim}
\end{minipage}

\textbf{Retrieved Chunk 6: } \\
\begin{minipage}[t]{0.45\textwidth}
\footnotesize
\begin{verbatim}
[0.901, -0.945, 0.198...]
\end{verbatim}
\end{minipage}

\textbf{Retrieved Chunk 7: } \\
\begin{minipage}[t]{0.45\textwidth}
\footnotesize
\begin{verbatim}
[0.012, -0.956, 0.109...]
\end{verbatim}
\end{minipage}

\textbf{Retrieved Chunk 8: } \\
\begin{minipage}[t]{0.45\textwidth}
\footnotesize
\begin{verbatim}
[0.123, -0.967, 0.210...]
\end{verbatim}
\end{minipage}

\textbf{Retrieved Chunk 9: } \\
\begin{minipage}[t]{0.45\textwidth}
\footnotesize
\begin{verbatim}
[0.234, -0.978, 0.321...]
\end{verbatim}
\end{minipage}

\textbf{Retrieved Chunk 10: } \\
\begin{minipage}[t]{0.45\textwidth}
\footnotesize
\begin{verbatim}
[0.345, -0.989, 0.432...]
\end{verbatim}
\end{minipage}

\textbf{Retrieved Chunk 11: } \\
\begin{minipage}[t]{0.45\textwidth}
\footnotesize
\begin{verbatim}
[0.456, -0.990, 0.543...]
\end{verbatim}
\end{minipage}

\textbf{Retrieved Chunk 12: } \\
\begin{minipage}[t]{0.45\textwidth}
\footnotesize
\begin{verbatim}
[0.567, -0.991, 0.654...]
\end{verbatim}
\end{minipage}

\textbf{Retrieved Chunk 13: } \\
\begin{minipage}[t]{0.45\textwidth}
\footnotesize
\begin{verbatim}
[0.678, -0.992, 0.765...]
\end{verbatim}
\end{minipage}

\textbf{Retrieved Chunk 14: } \\
\begin{minipage}[t]{0.45\textwidth}
\footnotesize
\begin{verbatim}
[0.789, -0.993, 0.876...]
\end{verbatim}
\end{minipage}

\textbf{Retrieved Chunk 15: } \\
\begin{minipage}[t]{0.45\textwidth}
\footnotesize
\begin{verbatim}
[0.890, -0.994, 0.987...]
\end{verbatim}
\end{minipage}

\textbf{Retrieved Chunk 16: } \\
\begin{minipage}[t]{0.45\textwidth}
\footnotesize
\begin{verbatim}
[0.901, -0.995, 0.098...]
\end{verbatim}
\end{minipage}

\textbf{Retrieved Chunk 17: } \\
\begin{minipage}[t]{0.45\textwidth}
\footnotesize
\begin{verbatim}
[0.012, -0.996, 0.209...]
\end{verbatim}
\end{minipage}

\vspace{5mm}
\textit{Note: The above chunks are retrieved with respect to query embedding; [0.321, -0.654, 0.789...] by hybrid retriever and then done RRF on it.}
\end{tcolorbox}

We then decode each chunk into its string format and concatenate them to serve as context for generating SOAP notes.

\begin{tcolorbox}[colback=blue!5!white,colframe=blue!75!black,title=Retrived information from the Patient-Doctor Conversation which is Relevent for Generating SOAP Notes, breakable]
\footnotesize
I've had a cough for about six months. Recently, I've noticed some blood. Is it a dry or wet cough? It's mostly dry. But lately, there's been some blood. How much blood are you coughing up? About two or three teaspoons a day. Any shortness of breath or chest pain? Yes, there's shortness of breath, especially with activity. But no chest pain. Any recent weight loss? Yes, around ten to fifteen pounds in the last two months. Do you smoke? Yes, half a pack a day. I've been cutting down. We need to do a chest X-ray and sputum test. Lung cancer is a concern given your symptoms and smoking history.
\end{tcolorbox}

\subsection*{Inference}

We then pass the output from the retriever-based filtering, along with the LLM query, to the LLM (whether fine-tuned or not) to generate the SOAP notes.

\begin{tcolorbox}[colback=blue!5!white,colframe=blue!75!black,title=SOAP Note]
\footnotesize
\textbf{Subjective:} \\
- Chief Complaint: Persistent cough for six months, with recent onset of blood in sputum \\
- Cough: Mostly dry, with blood present (approximately two to three teaspoons daily) \\
- Shortness of Breath: Noted, particularly with activity \\
- Chest Pain: None reported \\
- Weight Loss: Significant loss of 10-15 pounds over the past two months \\
- Smoking History: Current smoker, approximately half a pack per day; attempting to reduce \\

\textbf{Objective:} \\
- General Appearance: Weight loss evident \\
- Respiratory: Dry cough with recent hemoptysis. Shortness of breath noted on exertion \\
- Vital Signs: [To be completed based on actual values] \\
- Physical Exam: [To be completed based on findings, if available] \\

\textbf{Assessment:} \\
- Primary Concern: Hemoptysis with chronic cough, significant weight loss, shortness of breath, and smoking history raise concern for possible lung cancer \\
- Differential Diagnosis: Lung cancer, chronic bronchitis, tuberculosis, or other respiratory pathology \\

\textbf{Plan:} \\
- Immediate Actions: \\
  - Order Chest X-ray to assess for possible malignancy or other abnormalities \\
  - Request Sputum Test to evaluate for infectious or malignant cells \\
- Follow-Up: Schedule a follow-up appointment to review test results and determine further management \\
- Patient Education: Discuss the importance of smoking cessation and provide resources for support in quitting \\
\end{tcolorbox}

\captionof{figure}{An example of a SOAP note summarizing patient symptoms and management plan.}
\label{box:soap_note}
    

==> abstract.tex <==
This is the abstract page...

==> data.tex <==
%https://aclanthology.org/2023.eacl-main.168.pdf---MTS dataset 

==> data_stat_MTS-dialog.tex <==
\begin{table}[ht]
\centering
\caption{Statistics of the MTS-Dialog Dataset.}
\label{mts_dialog_data_stats}
\renewcommand{\arraystretch}{1.30}%
\begin{tabular}{lllll}
\hline
\multicolumn{5}{c}{\textbf{Patient-Doctor Conversation}}                                                                                     \\ \hline
\multicolumn{1}{l|}{}      & \multicolumn{1}{l|}{\textbf{Sentences}} & \multicolumn{1}{l|}{\textbf{Words}} & \multicolumn{1}{l|}{\textbf{Tokens}} & \textbf{Vocabulary} \\ \hline
\multicolumn{1}{l|}{count} & \multicolumn{1}{l|}{}          & \multicolumn{1}{l|}{}      & \multicolumn{1}{l|}{}          &            \\ \hline
\multicolumn{1}{l|}{mean}  & \multicolumn{1}{l|}{}          & \multicolumn{1}{l|}{}      & \multicolumn{1}{l|}{}          &            \\ \hline
\multicolumn{1}{l|}{max}  & \multicolumn{1}{l|}{}          & \multicolumn{1}{l|}{}      & \multicolumn{1}{l|}{}          &            \\ \hline
\multicolumn{1}{l|}{min}  & \multicolumn{1}{l|}{}          & \multicolumn{1}{l|}{}      & \multicolumn{1}{l|}{}          &            \\ \hline
\end{tabular}
\end{table}

==> himanshu_background.tex <==
\subsection{SOAP (Subjective, Objective, Assessment, Plan) Notes}
SOAP (Subjective, Objective, Assessment, Plan) notes are a structured method for documenting patient encounters in various healthcare settings, essential for ensuring clear communication among healthcare providers and maintaining comprehensive medical records. The SOAP note format was developed by Dr. Lawrence Weed in the late 1960s \cite{weed1993medical} as part of the Problem-Oriented Medical Record (POMR) system, aiming to improve the organization and clarity of medical documentation. Widely adopted in medical, pharmacy, and general practice education, the format has largely remained consistent, though some modifications have been made to adapt to specific specialties and electronic health records (EHRs), reflecting the evolving needs of modern healthcare.

\begin{enumerate}
    \item \textbf{Subjective (S)}
    \begin{itemize}
        \item Includes the patient's verbal descriptions of their symptoms, history, and other relevant information. This section captures the patient's perspective, including their chief complaint, history of present illness, past medical history, family history, social history, and review of systems \cite{santiago2016soap}.
        \item In pharmacy practice, the subjective section may also include medication history, patient concerns, and reports of adverse events \cite{sando2017assessment}.
    \end{itemize}

    \item \textbf{Objective (O)}
    \begin{itemize}
        \item Consists of measurable and observable data obtained through physical examination, laboratory tests, and other diagnostic procedures. This includes vital signs, physical exam findings, laboratory data, and current medications \cite{seo2016pilot}.
        \item There is variability in how objective data are documented, but it generally includes vital signs, physical exam information, laboratory data, and medications \cite{sando2017assessment}.
    \end{itemize}

    \item \textbf{Assessment (A)}
    \begin{itemize}
        \item Involves the healthcare provider's clinical judgment regarding the patient's condition. This section includes a diagnosis or differential diagnosis and an evaluation of the patient's progress \cite{sando2017assessment}.
        \item Common elements in the assessment section for pharmacists include identifying drug-related problems (DRPs), goals of therapy, and the rationale for the assessment. Priority ordering of DRPs may also be included \cite{seo2016pilot}.
    \end{itemize}

    \item \textbf{Plan (P)}
    \begin{itemize}
        \item Outlines the proposed management and treatment plan for the patient. This includes specific drug therapy recommendations, non-drug therapy, monitoring parameters, patient education, and follow-up instructions \cite{santiago2016soap}.
        \item The plan should specify adjustments to medication regimens, monitoring for efficacy and toxicity, patient education, and follow-up care \cite{sando2017assessment}.
    \end{itemize}
\end{enumerate}

SOAP notes are essential in healthcare for enhancing communication, ensuring comprehensive documentation, improving patient care, and serving as an educational tool. They provide a standardized format that ensures all healthcare providers have a consistent understanding of a patient's status, treatment plan, and progress, which is vital in multi-provider settings. The structured documentation aids in making informed clinical decisions, tracking patient progress, and maintaining continuity of care \cite{seo2016pilot}. Additionally, SOAP notes create a thorough record for legal purposes and quality assurance, and they are invaluable for teaching students and trainees how to document clinical encounters systematically and comprehensively.

However, maintaining SOAP notes can be challenging due to the time-consuming nature of writing detailed documentation, especially in busy clinical settings with limited patient interaction time. Healthcare providers must balance engaging with patients and accurately documenting encounters, which can disrupt the flow of conversation and add to their cognitive load. This dual tasking can lead to documentation errors or omissions and interrupt the natural workflow of patient care, making it difficult to maintain a seamless interaction with patients. Despite their importance, maintaining SOAP notes can be challenging for doctors. The process requires meticulous attention to detail and can be time-consuming, particularly in busy clinical settings where doctors must balance documentation with patient care. The need to accurately capture subjective patient statements, objective clinical findings, assessments, and detailed plans for treatment can be overwhelming. Additionally, the pressure to maintain thorough and accurate records while managing a high patient volume can lead to stress and potential burnout among healthcare providers. This challenge is compounded when there are inconsistencies in the elements evaluated within each section of the SOAP notes, leading to variability in documentation practices across different institutions and practitioners \cite{wu2021recursively}.

\subsection{Large Language Models (LLMs)}
Large Language Models (LLMs), such as GPT-4, LLAMA3, and PaLM, represent the cutting edge of computational linguistics. They are built upon Transformer architectures, a neural network framework introduced by Vaswani et al. in 2017, known for its efficiency in processing and generating sequences of data through a self-attention mechanism \cite{vaswani2017attention}. This self-attention mechanism allows Transformers to manage and interpret dependencies between different parts of the input text, making them particularly well-suited for tasks in Natural Language Processing (NLP).

Transformers have revolutionized NLP by enabling models to understand and generate human language more effectively. LLMs typically have vast parameter spaces, often comprising hundreds of billions of parameters, which allow them to capture the complexities and nuances of language. The core of their functionality lies in the self-attention mechanism, which helps them understand the context and relationships within the text, leading to more accurate and relevant outputs.

There are different Transformer architectures that LLMs use, each with specific strengths:

\begin{enumerate}
    \item \textbf{Decoder-Only Models: }These models generate output based solely on a given context or prompt. They do not transform the input data into a new representation but instead focus on generating text that follows logically from the prompt e.g., GPT-2, GPT-3.

    \item \textbf{Encoder-Only Model: }These models generate output based solely on a given context or prompt. They do not transform the input data into a new representation but instead focus on generating text that follows logically from the prompt e.g., GPT-2, GPT-3.

    \item \textbf{Decoder-Only Models: }These models process and transform input data into a fixed representation, which can then be used for various downstream tasks like classification or sentiment analysis. They excel at understanding and encoding the input text e.g., BERT, RoBERTa.

    \item \textbf{Encoder-Decoder Architectures: }These combine both encoding and decoding processes. The encoder transforms the input into a representation, which the decoder then uses to generate output. This architecture is powerful for tasks that require transforming input text into a different format or language, such as translation or summarization e.g., BART.
\end{enumerate}

LLMs also incorporate advanced techniques like prompting or in-context learning, where they generate text based on the context provided within the input. This approach enhances the relevance and coherence of the generated text, making LLMs highly effective for interactive tasks such as question-and-answer sessions \cite{chang2024survey}.

Insights from studies such as \cite{tripathi2023experimental} reveal how language models such as BERT establish relationships between expressions and queries, shedding light on chatbot interaction styles and response quality. This study contributes to understanding how advanced language models can be integrated into chatbots for more nuanced and context-aware responses. These insights pave the way for exploring how combining these models with other techniques, much like querying information from a well-organized document, can unlock even greater potential in language understanding and generation.

\subsection{Retrieval-Augmented Generation (RAG)}
RAG is an advanced text generation paradigm that merges deep learning technology with traditional retrieval techniques to enhance the performance of various natural language processing (NLP) tasks \cite{li2022survey, zhao2024retrieval}. By retrieving relevant information from external data sources based on the input query, RAG incorporates this data into the text generation process, improving both the quality and accuracy of the generated text \cite{zhao2024retrieval}. Key components include a retriever, which extracts pertinent information using methods like sparse-vector retrieval, dense-vector retrieval, and task-specific retrieval, and a generator that uses this retrieved information as additional context to produce the target text (RAG). Models such as RAG-Sequence and RAG-Token enable different strategies for integrating the retrieved data, allowing flexibility in how the information is used during generation \cite{lewis2020retrieval}.

Building on this foundational approach, RAG has been successfully applied across various domains, including dialogue systems, machine translation, summarization, and text style transfer. In knowledge-based question answering, RAG enhances open-domain QA by incorporating external knowledge bases \cite{lewis2020retrieval, li2022survey, zhao2024retrieval}, while in multi-modal applications such as image captioning, video QA, and 3D text generation, it demonstrates remarkable versatility. Enhancements like adaptive retrieval, which dynamically decides the necessity of retrieval based on query complexity, and iterative RAG, which refines results through repeated cycles of retrieval and generation, further improve content quality and address knowledge gaps.

However, despite its successes, RAG faces challenges such as retrieval sensitivity and efficiency. The performance of RAG models is highly dependent on the quality of retrieved documents, necessitating improved retrieval methods to ensure high relevance and quality \cite{li2022survey, zhao2024retrieval}. Balancing retrieval memory size with efficiency is also crucial to reduce overhead and enhance inference speed \cite{li2022survey}. Future research directions include extending retrieval-based generation to multi-modal tasks involving data from different modalities and developing customized metrics for retrieval to enhance control over text generation and improve diversity in retrieval results. Overall, RAG represents a significant advancement in text generation, offering improved performance and adaptability across a wide range of applications. As research continues to address its current limitations, RAG's potential for broader and more effective applications in NLP and beyond is substantial, promising further innovations and improvements in the field \cite{zhao2024retrieval}.

==> hyper_param_table.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{graphicx}
% \begin{table*}[ht]
% \centering
% \footnotesize
% \caption{An overview of Hyper-parameters used to fine-tune PLM in \framework. }
% \label{hyperparams_ft}
% \resizebox{\textwidth}{!}{%
% \begin{tabular}{l|l|l}
% \hline
% \textbf{Hyperparameter}         & \textbf{Value} & \textbf{Summary}                                      \\ \hline
% max\_seq\_length                & 2048           & truncate output sequences to this max length          \\ %\hline
% prompt                          & alpaca prompt \ref{alpaca_prompt}  & instruction text prepended to all inputs              \\ %\hline
% r                               & 16             & rank of the low-rank adaptation matrices              \\ %%\hline
% lora\_alpha                     & 16             & scaling factor applied                                \\ %\hline
% lora\_dropout                   & 0              & 0 indicate all weights are considered                 \\ %\hline
% packing                         & FALSE          & each example is treated independently during training \\ %\hline
% bias                            & none           & restrics additional bias in LORA layers               \\ %\hline
% per\_device\_train\_batch\_size & 2              & the batch size for training per device                \\ %\hline
% gradient\_accumulation\_steps   & 4              & \# of steps to accumulate gradientsin traning         \\ %\hline
% use\_gradient\_checkpointing    & TRUE           & enables gradient checkpointing                        \\ %\hline
% warmup\_steps                   & 5              & number of warmup steps during training                \\ %\hline
% num\_train\_epochs              & 3              & model will train on the dataset three times           \\ %\hline
% lr\_scheduler\_type             & linear         & linear scheduler decreases the learning rate linearly \\ %\hline
% fp16                            & TRUE           & whether to use FP16 during training                   \\ %\hline
% learning\_rate                  & 0.0002         & learning rate during training                         \\ %\hline
% logging\_steps                  & 1              & specifies traning log will be recored once            \\ %\hline
% optim                           & adamw\_8bit    & optimizer used during training                        \\ %\hline
% weight\_decay                   & 0.01           & weights will be slightly penalized during training    \\ %\hline
% seed                            & 3407           & sets the random seed for reproducibility              \\ \hline
% \end{tabular}%
% }
% \end{table*}


\begin{table}[ht]
\centering
\scriptsize
\caption{An overview of Hyper-parameters used to fine-tune PLM in \framework. }
\label{hyperparams_ft}
\begin{tabular}{l|l|p{3.5cm}}
\hline
\textbf{Hyperparameter}         & \textbf{Value} & \textbf{Summary}                                      \\ \hline
max\_seq\_length                & 2048           & truncate output sequences to this max length          \\ %\hline
prompt                          & alpaca prompt & instruction text prepended to all inputs              \\ %\hline
r                               & 16             & rank of the low-rank adaptation matrices              \\ %\hline
lora\_alpha                     & 16             & scaling factor applied                                \\ %\hline
lora\_dropout                   & 0              & 0 indicates all weights are considered                \\ %\hline
packing                         & FALSE          & each example is treated independently during training \\ %\hline
bias                            & none           & restricts additional bias in LORA layers              \\ %\hline
per\_device\_train\_batch\_size & 2              & batch size for training per device                    \\ %\hline
gradient\_accumulation\_steps   & 4              & \# of steps to accumulate gradients in training       \\ %\hline
use\_gradient\_checkpointing    & TRUE           & enables gradient checkpointing                        \\ %\hline
warmup\_steps                   & 5              & number of warmup steps during training                \\ %\hline
num\_train\_epochs              & 3              & model will train on the dataset three times           \\ %\hline
lr\_scheduler\_type             & linear         & linear scheduler decreases learning rate linearly     \\ %\hline
fp16                            & TRUE           & whether to use FP16 during training                   \\ %\hline
learning\_rate                  & 0.0002         & learning rate during training                         \\ %\hline
logging\_steps                  & 1              & specifies training log will be recorded once          \\ %\hline
optim                           & adamw\_8bit    & optimizer used during training                        \\ %\hline
weight\_decay                   & 0.01           & weights will be slightly penalized during training    \\ %\hline
seed                            & 3407           & sets the random seed for reproducibility              \\ \hline
\end{tabular}
\end{table}


==> method.tex <==
%\hl{wip---target to finish by 20th---Subash}
\subsection{Retriever Based Filtering}

The first module in our \framework is designed to systematically process doctor-patient conversation transcripts to extract relevant information necessary for generating SOAP clinical summaries. Initially, the module receives the raw transcripts from the interactions between doctors and patients. For a given retrieval prompt (query)  $r_p$, the first module mainly consists of three component \textbf{1) Splitting}: Let $T$ be the raw transcript $T$. The transcript is a sequence of sentences with punctuation, expressed as: 

\hl{Subash---wip}
\[T= \{s_1,s_2,...,s_n\}\] where $s_i$ represents a sentence or puncutation mark in the transcript, and $n$ is the total number of words and punctuation marks in $T$. To split $T$ into sentences we apply regular expressions to detect sentence boundaries. Specifically, it targets periods (.), question marks(?), and exclamation (!), which denote the end of a sentence. Let $B$ be the set of boundary indices where a sentence ends such that:
\[B = \{i|w_i \textit{ is a } period(.) \textit{ or } question mark(?) \textit{ or } exclamation(!) \}\] 
The tanscript $T$ is then split into $n$ sentences (chunks) based on the boundaries detected by the regular expression. Let each chunk be represented by $C_i$, where $i$ ranges from 1 ro $n$. Each sentence $C_i$ is formed by collecting the words from  $T$ between boundary indices $B_{i-1}$  and $B_i$: \[ S_i = \{w_j|B_{i-1} < j \leq B_i\}\] Consequently, the transcript $T$ is split into $n$ chunks:
\[Chunks (T)= \{C_1,C_2,...,C_n\}\]

\textbf{(2) Indexing}
Given the chunks of Transcripts $T =\{C_1,C_2,...,C_n\} $, where $c_i$ represents the document chunk. Indexing is the process of converting $c_i$ into vectors through an embedding model $f_e(.)$, and then store vectors in vector database.  

\begin{equation}
\begin{aligned}
&\mathcal{I}=\left\{e_1, e_2, \ldots, e_n\right\} \quad \text { and } \quad e_i=f_e\left(c_i\right) \in \mathbb{R}^d\\
&\text { }
\end{aligned}
\end{equation}

\textbf{(3) Retrieval} Transform the retriever prompt $r_{p}$ using same encoding model such that $r_p = f_e(r_p)$ and then filter out the top $k$ document chunks. The retrieval process uses an ensemble method that combines sparse retriever (for example BM25) and dense retriever (for example DPR), assigning different weights to each, then ranks it using ranking algorithm. Sparse retriever measures the relevance of the chunk $c_i$ to the retriever prompt $r_{p}$ based on term frequency and document frequency. 
The sparse retriever can be expressed as: 
\begin{equation}
    \mathcal{R}_{sparse} = top{_k} (\{(r_p, e_i) |e_i \in I\})\rightarrow S^{r_{p}}
\end{equation}
 where $S^{r_{p}} = \{S_{d1},S_{d2},...,S_{dk}\}$ represents the relevant document retrieved by sparse retriever. Whereas dense retriever retrieves top document using similarity measure and it can be expressed as:
\begin{equation}
\begin{aligned}
&\mathcal{R}_{dense} = \underset{c_i \in T}{\operatorname{top_k}} \operatorname{Sim}\left(\{(r_p, e_i) |e_i \in I\}\right) \rightarrow D^{r_{p}}\\
&\text {}
\end{aligned}
\end{equation}
where $D^{r_{p}} = \{D_{d1},D_{d2},...,D_{dk}\}$ represents the relevant documents for retriever prompts ${r_{p}}$. The similarity function $Sim(.)$ is cosine similarity such that: 

\begin{equation}
\begin{aligned}
&\operatorname{Sim}\left({r_{p}}, c_i\right)=\quad \frac{e_{r_{p}} \cdot e_{c_i}}{\left\|e_{r_{p}}\right\| \cdot\left\|e_{c_i}\right\|}\\
&\text {}
\end{aligned}
\end{equation}

 % \begin{equation}
 %     Dense(R_p, v_i) = cos(v_{r_p}, v_i)
 % \end{equation}
 % $Dense(R_p, v_i) = cos(v_{r_p}, v_i)$ where, $v_i$ is embedding vector of chunk $S_i$ and $v_{r_p}$ is embedding vector of retrieval prompt. 
%  The ensemble score $ens(R_p,s_i)$ for chunk $s_i$ is weighted sum of sparse and dense retriever scores: 
% \begin{equation}
% \operatorname{ens}\left(R_p, s_i\right)=w_{b} \cdot \mathcal{R}_{sparse}+w_{\text {d }} \cdot \mathcal{R}_{dense}
% \end{equation}

% The ensemble retriever ranks the chunks based on the ensemble score:
% \begin{equation}
% \left\{s_{i_1}, s_{i_2}, \ldots, s_{i_k}\right\}=\operatorname{Rank}\left(\left\{\operatorname{Ens}\left(R_p, s_i\right)\right\}_{i=1}^m\right)
% \end{equation}

%Each retrieval method produces ranked list of chunks based on their relevance to the retrieval prompt. 

For each method we assign weighted score threshold 


For each chunk $S_i$, each method assigns rank, where the rank is the position of the chunk in the ranked list (1 for most relevant, 2 for the next most relevant, etc.). 

The top $k$ chunks with highest ensemble scores are returned as the result for the retrieval prompt $R_p$. This is then passed to next phase for generation.

% that are most similar based on vector similarity. 

% \begin{equation}
% \begin{aligned}
% &\mathcal{R}: \underset{s_i \in T}{\operatorname{topk}} \operatorname{Sim}\left(R_{pi}, s_i\right) \rightarrow D^{R_{pi}}\\
% &\text {}
% \end{aligned}
% \end{equation}





%This procedure employs regular expressions to detect sentence boundaries, specifically targeting periods and question marks. As a result, each identified sentence is isolated and treated as a distinct chunk for further processing. Next, these chunks undergo an embedding generation process. This step involves applying embedding models to transform the textual chunks into corresponding embedding vectors. These embedded vectors encapsulate the semantic content of the sentences, making them suitable for further analysis. Subsequently, an advanced retriever mechanism analyzes the embedded chunks using a structured prompt designed to extract SOAP (Subjective, Objective, Assessment, and Plan) information. The retriever processes the chunks, extracting clinically relevant vectors, which are then filtered to remove noise and irrelevant data, ensuring the retention of pertinent information.

%The filtered vectors are converted back into coherent text through a process called text reconstruction. The reconstructed texts are concatenated to form a combined text document, serving as input context for the inference module.

\subsection{Inference}
The input to the inference module includes the patient context, derived from the retriever-based filtering module, and a prompt. This prompt instructs a fine-tuned PLM to generate clinical summaries in a 0-shot setting based on the provided context. The inference module leverages the fine-tuned PLM which we refer to as generator. %, which has been pre-trained to produce SOAP summaries. By processing the structured prompt and patient context, the model generates a coherent and comprehensive clinical SOAP summary, ensuring the extraction of clinically relevant information from patient context. 
\framework is effective in zero-shot settings due to the fine-tuning of the PLM, allowing it to generalize well to new, unseen patient contexts without requiring additional training data.

\subsubsection{Fine-tuning}
In this paper, we opt for Parameter Efficient Fine Tuning \cite{} approach to finetune a PLM for clinical summary generation. PEFT allows one to fine tune models with minimal resources and costs. We adopt LoRA (Low Rank Adaptation) \cite{} method and load pre-trained models in GPU as quantized 4-bit weights. The reason for this choice of ours is because  we wanted to investigate the 1. feasibility of training PLM such as LLAMA-3 on single consumer GPU with 24GB memory (e.g. Nvidia 4090 ) 2. effectiveness of fine-tuned PLM with 4-bit precision in accurately generating clinical summaries.  On the other hand,  PEFT also prevents \emph{catastrophic forgetting} after the model has been trained \cite{}.  We follow alpaca prompt \cite{} for both fine-tuning and inference task. An illustration of Alpaca prompt is depicted in Fig \ref{alpaca_prompt}. The training is supervised fine tuning. The dataset used for fine-tuning is discussed in Section \ref{data_section}. The hyper-parameters of training can be seen on Appendix \ref{appendix}. 
\input{aplaca_prompt}
\subsubsection{Summary Generation}
After getting the relevant documents. The retriever prompt $R_p$ and the retrieved document based on  $R_p$ which is $D^{R_p}$ chunks are inputted together to the fine-tuned PLM to generate the final answer, where $\mathcal{F}_{  \mathcal{P} \mathcal{L} \mathcal{M}}$ is a fine-tuned PLM and [·, ·] stands for concatenation.
\begin{equation}
y= \mathcal{F}_{  \mathcal{P} \mathcal{L} \mathcal{M}} \left(\left[D^{R_p}, R_p\right]\right)
\end{equation}

Inference is performed on zero-shot settings. An example of final clinical summary for a specific patient-doctor conversation can be seen in Appendix \ref{appendix}. 



% \begin{figure*}
%   \centering
%   \includegraphics[width=.75\linewidth]{figs/Soap_final.pdf}
%   \caption{A proof-of-concept architecture showcasing the possibility of generating a semi-structured clinical summary in SOAP format. }
%   \label{fig:soap_summaries}
% \end{figure*}

==> old_edit.tex <==
%\hl{wip---target to finish by 20th---Subash}

This section presents the architecture of our framework, \framework, and outlines our methodology. The framework consists of two main modules: \emph{retriever-based filtering} and \emph{inference}, as illustrated in Fig. \ref{fig:soap_summaries}. The following subsections provide a detailed explanation of each module.
\subsection{Retriever-based Filtering}
\hl{WIP---subash}
The first module in our framework systematically processes doctor-patient conversation transcripts to extract the subjective, objective, assessment, and plan components from each interaction. An example of retrieval prompt (query) $Q_R$, is \emph{``Extract subjective, objective, assessment, and plan details from a given transcript''}. For extraction this module utilizes the following three components:

\textbf{(1) Splitting:} Splitting is the process of converting each sentence in the transcript into chunks.
% using $Chunk$ function such that:
% \begin{equation*}
%     Chunk(S) = \{S^{p_{i + 1}}_{p_i} | 1 \leq p_i < p_{i + 1} \leq n \text{ and } S_{p_i} \in D\}
% \end{equation*}

% \noindent where, $S = \{s_1, s_2, s_3, \cdots s_n\}$ is a string where $s_i \in \sum$ (a finite set of characters), $D = \{ . , ?, ! \}$ is the set of delimiters, and $p_i, p_{i + 1}$ are consecutive positions in $\{ i | 1 \leq i \leq n \text{ and } s_i \in D\}$. The $Chunk$ function splits a string $S$ into substrings, each ending with a delimiter from $D$. Each resulting chunk is a segment of the original string that includes one of these delimiters. Given a raw transcript $T$, applying $Chunk(T)$ will split the transcript into individual sentences based on the delimiters $D$.


\hl{previous expression }
Let $T$ be the raw transcript. The transcript is a sequence of words and punctuation marks, expressed as: $ T = \{s_1, s_2, \dots, s_n\}$ where each $s_i$ represents a word or punctuation mark, and $n$ is the total number of words and punctuation marks in $T$. To split $T$ into sentences, we apply regular expressions to detect sentence boundaries. Specifically, we target periods (.), question marks (?), and exclamation marks (!), which denote the end of a sentence. Consequently, the transcript $T$ is split into chunks:
\[
T = \{C_1, C_2, \dots, C_{n}\}
\]


% Let $B$ be the set of boundary indices where a sentence ends, such that:

% \[
% B = \{i \ | \ s_i \text{ . or ? or !) }\}
% \]

% The transcript $T$ is then split into sentences based on the boundaries detected by the regular expression. Let each chunk be represented by $C_i$, where $i$ ranges from $1$ to $|B|$. Each chunk $C_i$ is formed by collecting the words and punctuation marks from $T$ between boundary indices $B_{i-1}$ and $B_i$:

% \[
% C_i = \{s_j \ | \ B_{i-1} < j \leq B_i \}
% \]



% \begin{itemize}
%     \item $S = \{s_1, s_2, s_3, \cdots s_n\}$ is a string where $s_i \in \sum$ (a finite set of characters).
%     \item $D = \{ . , ?, ! \}$ set of delimiters.
%     \item $p_i, p_{i + 1}$ are consecutive positions in $\{ i | 1 \leq i \leq n \text{ and } s_i \in D\}$
% \end{itemize}


% Therefore, $Chunk$ function splits a string \textit{S} into substrings, where each substring ends with a delimiter \textit{(., ?, !)}, and the delimiter is included in the chunk. Each resulting chunk is a segment of the original string that includes one of the delimiters at the end.


 

% \begin{equation*}
%     Chunk(T) = \{ C_1, C_2, C_3 \cdots C_n \}
% \end{equation*}

%By splitting each sentence, we ensure that each chunk carries complete information on its own, making it independent of preceding or succeeding chunks for comprehension.

\textbf{(2) Indexing:} Given the chunks of transcripts, $\{C_1, C_2, \cdots, C_n\}$, where $C_i$ represents a document chunk, indexing is the process of converting $C_i$ into vectors through an embedding model $E$. These vector embedding can be stored into a vector database. To do so, first, we tokenize each chunk $C_i$ into tokens ${ t_1, t_2, t_3, \dots, t_k }$. Let $E_t$ represent the embedding function that maps each token of $t_j$ to its corresponding embedding vector using an embedding matrix M:

\begin{equation*} 
    e_{t_j} = E_t(t_j) = M[t_j] 
\end{equation*}

\noindent where, $M \in \mathbb{R}^{|V| \times d}$ is the embedding matrix, with $|V|$ being the size of the vocabulary and $d$ the embedding dimension, and $M[t_j]$ represents the row in the matrix $M$ corresponding to the token $t_j$, which gives the embedding vector $e_{t_j} \in \mathbb{R}^d$.


% It can then  and then store vectors in a vector database.
 % if we want persistent database.

% Here, we first tokenize each chunk $C_i$ into tokens $\{ t_1, t_2, t_3 \cdots, t_k \}$. Let $E_t$ be the embedding matrix. The embedding vector $t_j$ is:

% \begin{equation*}
%     e_{t_j} = E_t[t_j]
% \end{equation*}

%Now, we pass the token embeddings through the model to obtain hidden state vectors $H^L_{t_j}$  ($L$ is the total number of layers in the embedding model) for each token. Finally, using average pooling (reduceing the spatial dimensions of feature maps by dividing them into non-overlapping regions and computing the average value for each region, which helps in dimensionality reduction and retaining important features) to compute the final embedding of $C_i$:

% \begin{equation*}
%     E(C_i) = \frac{1}{k}\sum_{j=1}^{k}H_{t_j}^{L}
% \end{equation*}

% Therefore, when we pass $Chunk(T)$ into the embedding model, we get

% \begin{equation}
% \label{eq1}
%     E(Chunk(T)) = \{E(C_1), E(C_2), E(C_3), \cdots, E(C_n)\}
% \end{equation}

% In this step, we also embedd the retreiver prompt $Q_R$ as well.

% \begin{equation*}
%     Q_R' = E(Q_R)    
% \end{equation*}

% \begin{figure*}
%   %\centering
%   \includegraphics[width=.60\linewidth]{figs/Soap_final.pdf}
%   \caption{A graphical depiction of \framework's architecture. It comprises two moduels: \emph{retrieved-based filtering} and \emph{inference}. These module work in tandem to generate clinical summaries in SOAP format.}
%   \label{fig:soap_summaries}
%   \vspace{-3mm}
% \end{figure*}
\begin{figure*}
  %\centering
  \includegraphics[width=1\linewidth]{figs/final_archi.pdf}
  \caption{\textbf{A} is graphical illustration of the \framework architecture. It comprises two modules: \emph{retrieved-based filtering} and \emph{inference}. \textbf{B} represents patient-doctor conversation, and \textbf{C} represents generated clinical summary.}
  \label{fig:soap_summaries}
  \vspace{-3mm}
\end{figure*}


Next, we pass the token embeddings through the model to obtain hidden state vectors $H^L_{t_j}$ for each token, where $L$ is the total number of layers in the embedding model. Finally, we apply average pooling—a technique that reduces the spatial dimensions of feature maps by dividing them into non-overlapping regions and computing the average value for each region, which aids in dimensionality reduction while retaining important features. This process yields the final embedding of each chunk $C_i$:

\begin{equation*} E(C_i) = \frac{1}{k}\sum_{j=1}^{k}H_{t_j}^{L} \end{equation*}

Thus, when we pass $Chunk(T)$ into the embedding model, we obtain:

\begin{equation} \label{eq1} E(Chunk(T)) = {E(C_1), E(C_2), E(C_3), \dots, E(C_n)} \end{equation}

\noindent In this step, we also embed the retrieval prompt $Q_R$ such that:

\begin{equation*} Q_R' = E(Q_R)
\end{equation*}

%Embeddings are crucial in retrieval tasks because they map data into a continuous vector space where semantically similar items are close together. This allows for a deeper understanding of the content beyond exact keyword matches. By reducing dimensionality and preserving important features, embeddings improve retrieval efficiency and accuracy. They also handle variability in data and enable scalable search through efficient indexing. Advanced embeddings capture contextual information, further enhancing the relevance of search results.

\textbf{(3) Retrieval:} The retrieval process uses an ensemble method that combines sparse retriever (for example BM25 \cite{robertson1995okapi}) and dense retriever (for example DPR \cite{karpukhin2020dense}), assigning different weights to each ($W_{Sparse}$, and $W_{Dense}$), then ranks it using ranking algorithm. For our use case we implemented Reciprocal Rank Fusion (RRF) \cite{cormack2009reciprocal} which combines rankings from multiple sources by computing reciprocal rank scores. 

A sparse retriever searches for documents based on exact matches or specific token overlaps in a vector space, usually employing traditional keyword-based methods or indexing techniques. A sparse retriever ($R_{Sparse}$) can be represented as:
\begin{equation*}
    R_{Sparse}(E(C_i), Q_R') = TF-IDF(E(C_i), Q_R')
\end{equation*}
where, TF-IDF (Term Frequency-Inverse Document Frequency) measures how well terms in the document match the query (\emph{retriever prompt in our case})) terms. The output of $R_{Sparse}(E(C_i), Q_R')$ is a list of chunks with their corresponding ranks $Rank_{Sparse}(E(C_i))$:

\begin{equation*}
\begin{aligned}
R_{Sparse} = \{ (E(C_1), Rank_{Sparse}(E(C_1))),\\ (E(C_2), Rank_{Sparse}(E(C_2))),\\ \cdots, \\(E(C_{n_{Sparse}}), Rank_{Sparse}(E(C_{n_{Sparse}}))) \}
\end{aligned}
\end{equation*}
$Rank_{Sparse}(E(C_i))$ calculated using TF-IDF or similar methods. 

A dense retriever searches for documents based on the similarity of embedded vectors in a continuous vector space, using dense representations from models like BERT or GPT. A dense retriever ($R_{Dense}$) can be represented as:

\begin{equation*}
R_{Dense}(C_i, Q_R') = Sim(E(C_i), Q_R')
\end{equation*}

where $Sim$ denotes a similarity function, such as cosine similarity:

\begin{equation*}
Sim(E(C_i), Q_R') = \frac{\|E(C_i)\| \|Q_R'\|}{E(C_i) \cdot Q_R'}
\end{equation*}

 The output of $R_{Dense}(E(C_i), Q_R')$ is a list of chunks with their corresponding ranks $Rank_{Dense}(E(C_i))$:

\begin{equation*}
\begin{aligned}
R_{Dense} = \{ (E(C_1), Rank_{Dense}(E(C_1))),\\ (E(C_2), Rank_{Dense}(E(C_2))),\\ \cdots, \\(E(C_{n_{Dense}}), Rank_{Dense}(E(C_{n_{Dense}}))) \}
\end{aligned}
\end{equation*}

Where $Rank_{Dense}(E(C_i))$ represents the rank based on similarity score.

\begin{equation*}
    \begin{aligned}
        Docs_{Sparse} = sort(R_{Sparse}, by = Rank_{Sparse}(E(C_i)),\\ order = descending)[:W_{Sparse} \times R_{Sparse}]\\\text{and}\\Docs_{Dense} = sort(R_{Dense}, by = Rank_{Dense}(E(C_i)),\\ order = descending)[:W_{Dense} \times R_{Dense}]
    \end{aligned}
\end{equation*}

Next, we combine both $Docs_{Sparse}$ and $Docs_{Dense}$ to obtain the final set of embedded documents, before re-ranking them such that:
\begin{equation*}
    Docs = Docs_{Dense} \cup Docs_{Sparse}
\end{equation*}

The length of $Docs$ (say $m$) will be less then the total number of chunks created ($n$) i.e., $n_{Sparse} + n_{Dense} \geq m \leq n$. Once combined, we apply a ranking method to reorder the documents. This is done by using RRF algorithm.

\begin{equation*}
    Docs_{Ranked} = RRF(Docs) = \left[\frac{1}{Rank(E(C_j)) + b}\right]_{j=1}^m
\end{equation*}

Where $b$ is a bias to avoid division by zero, and $Rank(E(C_j))$ can be either  $Rank_{\text{Dense}}(E(C_j))$ or  $Rank_{\text{Sparse}}(E(C_j))$ depending on whether the document/embedded chunk is from $Docs_{\text{Dense}}$ or $Docs_{\text{Sparse}}$, respectively. If a document appears in both $Docs_{\text{Sparse}}$ and $Docs_{\text{Dense}}$ with different rankings, we sum the reciprocals of each rank from both retrievers. Typically $Rank(E(C_j)) \in [0, 1]$, this summed reciprocal score can exceed 1. This combined score is used for final ranking, with higher scores indicating greater relevance.% This approach reflects the consensus among retrievers, giving higher scores to documents ranked highly by multiple sources.

Finally, we decode (text reconstruction) the document back into individual sentences. This step reverts the document to the complete information consisting of the split sentences, or chunks, as described before in Equation \ref{eq1}. The final decoded output will include only those chunks that contain either the subjective, objective, assessment, or plan components from the given transcript.

\begin{equation*}
\begin{aligned}
    Decoder(Docs_{Ranked}) = Decoded_{Chunks} =\\ \{Decoded_{Chunks-1}, Decoded_{Chunks-2}, \cdots, \\Decoded_{Chunks-m}\}
\end{aligned}
\end{equation*}

After reconstructing the text, we use the $Concat$ function to combine the reconstructed chunks, forming the context for inference. This concatenated text is denoted as $Concatenated_{Chunks}$.%, representing the final coherent document used for further processing.

\begin{equation*}
    Concatenated_{Chunks} = Concat(Decoded_{Chunks})
\end{equation*}

{By passing the transcripts through the retriever-based filtering, we effectively reduce the tokens that do not correspond to the generation of SOAP notes, thereby abstracting unnecessary information before sending it for inference. This reduction in tokens not only helps \framework avoid the token overflow problem but also mitigates the inference model from hallucination.}

%A decoder is needed to transform abstract, encoded representations back into human-readable formats, such as text. It converts high-dimensional embeddings or encoded data into coherent, contextually appropriate outputs. This process is crucial for generating variable-length sequences and maintaining the information captured during encoding. Essentially, it ensures that the final output is interpretable and usable.

\subsection{Inference}
The inference module receives the patient context, derived from the  $Concatenated_{Chunks}$, along with an \emph{instruction} , and a \emph{prompt} $Q_{PLM}$ as shown in Fig. \ref{fig:soap_summaries}. The instruction guides the language model in performing its task. In our case, we utilize Alpaca prompt, as shown in Fig. \ref{fig:alpaca_prompt} as our instruction. On the other hand, prompt directs a fine-tuned PLM to produce clinical summaries in a zero-shot setting. The fine-tuned generator processes the prompt, patient context, and instructions to generate a comprehensive clinical SOAP summary. In the following subsections we describe our fine-tuning approach and then detail summary generation.

\subsubsection{Fine-tuning}
In this work, we leverage PEFT \cite{houlsby2019parameter} approach to fine-tune a PLM for clinical summary generation. PEFT enables efficient fine-tuning with minimal resources and costs. Specifically, we adopt Low Rank Adaptation (LoRA) \cite{hu2021lora} method and load pre-trained models onto a GPU as quantized 4-bit weights. Our motivation for this approach is two-folds: first, to explore the \textbf{feasibility} of training a PLM, such as LLAMA-3, on a single consumer GPU with 24GB of memory (e.g., Nvidia 4090), and second, to assess the \textbf{effectiveness} of fine-tuned PLMs with 4-bit precision in accurately generating clinical summaries. Additionally, PEFT helps prevent \emph{catastrophic forgetting}\cite{kirkpatrick2017overcoming} after the model has been trained \cite{meta}. We use the Alpaca prompt \cite{alpaca} for both fine-tuning and inference tasks, as illustrated in Fig. \ref{fig:alpaca_prompt}. The training is conducted using Supervised Fine-Tuning (SFT). More information on training dataset is provided in Section \ref{data_section}.
% , and the training hyper-parameters are detailed in Appendix \ref{fine-tuning-details}.




%The reason for this choice of ours is because  we wanted to investigate the  \textbf{1. feasibility} of training PLM such as LLAMA-3 on single consumer GPU with 24GB memory (e.g. Nvidia 4090) \textbf{2. effectiveness} of fine-tuned PLM with 4-bit precision in accurately generating clinical summaries.  On the other hand,  PEFT also prevents \emph{catastrophic forgetting} after the model has been trained \cite{meta}.  We follow alpaca prompt \cite{alpaca} for both fine-tuning and inference task. An illustration of Alpaca prompt is depicted in Fig \ref{alpaca_prompt}. The training is supervised fine-tuning. The dataset used for fine-tuning is discussed in Section \ref{data_section}. The hyper-parameters of training can be seen on Appendix \ref{appendix}. 
\input{aplaca_prompt}
\subsubsection{Summary Generation}

We utilize the output of the first module—the context, i.e., the decoded relevant chunks containing subjective, objective, assessment, and plan information from a given transcript—along with an instruction and a prompt as input to the inference module to generate a clinical summary. These input are concatenated and passed together to a fine-tuned PLM for summary generation, where $\mathcal{F}_{  \mathcal{P} \mathcal{L} \mathcal{M}}$ is a fine-tuned PLM that understand how to generate a clinical summaries, $Q_{\mathcal{PLM}}$ is a prompt (query), \emph{$inst$} denotes {instruction}  and \textit{``[.,.,.]"} stands for concatenation.  

\begin{equation*}
    \begin{aligned}
        Summary = \mathcal{F}_{PLM}([context, prompt, inst]) =\\ 
        \mathcal{F}_{PLM}([Concatenated_{Chunks}, Q_{\mathcal{PLM}}, inst])
    \end{aligned}
\end{equation*}

%Inference is conducted in a zero-shot setting because \framework utilizes a fine-tuned PLM to generate summaries. The fine-tuning enables \framework to generalize well to new, unseen patient contexts without requiring additional training data. 
Inference is conducted in a zero-shot setting using a fine-tuned PLM. The fine-tuning process equips the model to generalize effectively, allowing it to generate accurate clinical summaries even for new, unseen patient conversations without requiring additional few-shot examples. An example of the final clinical summary for a specific patient-doctor conversation is provided in Fig. \ref{fig:soap_summaries} (B) and (C) respectively.  
%Appendix section (Fig \ref{box:summary_from_conversation}). 

% Inference is performed on zero-shot settings. An example of final clinical summary for a specific patient-doctor conversation can be seen in Appendix \ref{appendix}. 


% \framework is effective in zero-shot settings due to the fine-tuning of the PLM, allowing it to generalize well to new, unseen patient contexts without requiring additional training data.

% The retriever prompt $R_p$ and the retrieved document based on  $R_p$ which is $D^{R_p}$ chunks are inputted together to the fine-tuned PLM to generate the final answer, where $\mathcal{F}_{  \mathcal{P} \mathcal{L} \mathcal{M}}$ is a fine-tuned PLM and [·, ·] stands for concatenation.
% \begin{equation}
% y= \mathcal{F}_{  \mathcal{P} \mathcal{L} \mathcal{M}} \left(\left[D^{R_p}, R_p\right]\right)
% \end{equation}



% \begin{equation*}
%     \begin{aligned}
%         SOAP = LLM(context, query) =\\ 
%         LLM(concat(Decoded_{Chunks}), Q_{LLM})
%     \end{aligned}
% \end{equation*}





